Decentralized Reinforcement Learning for Multi-Agent Multi-Resource Allocation via Dynamic Cluster Agreements

This paper addresses the challenge of allocating heterogeneous resources among multiple agents in a decentralized manner. Our proposed method, Liquid-Graph-Time Clustering-IPPO, builds upon Independent Proximal Policy Optimization (IPPO) by integrating dynamic cluster consensus, a mechanism that allows agents to form and adapt local sub-teams based on resource demands. This decentralized coordination strategy reduces reliance on global information and enhances scalability. We evaluate LGTC-IPPO against standard multi-agent reinforcement learning baselines and a centralized expert solution across a range of team sizes and resource distributions. Experimental results demonstrate that LGTC-IPPO achieves more stable rewards, better coordination, and robust performance even as the number of agents or resource types increases. Additionally, we illustrate how dynamic clustering enables agents to reallocate resources efficiently also for scenarios with discharging resources.

==> commands.tex <==
%% Abbreviations
\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}}

\newcommand{\x}{\texttimes\ }


%% Citations
\newcommand{\citeauthorcite}[1]{\citeauthor*{#1}~\cite{#1}}


%% Figures
% example: \fig{universe}{The Universe}
% reference later with: \figref{universe}
\newcommand{\fig}[3][0.45]{%
    \begin{figure}[!t]%
        \centering%
        \includegraphics[width=#1\textwidth]{#2}%
        \caption{#3}%
        \label{fig:#2}%
    \end{figure}%
}

\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}


%% Sub-figures
% example:
% \begin{subfigs}{label}{Title}
%   \subfig[0.45]{hands-none}{None}
%   \subfig[0.45]{hands-occlusion}{Occlusion}
% \end{subfigs}
% reference later with: \figref{label}
\NewDocumentEnvironment{subfigs}{m m}{%
    \begin{figure}[!t]%
        \centering%
        }{%
        \caption{#2}%
        \label{fig:#1}%
    \end{figure}%
}

\NewDocumentEnvironment{subfigswide}{m m}{%
    \begin{figure*}[!t]%
        \centering%
        }{%
        \caption{#2}%
        \label{fig:#1}%
    \end{figure*}%
}

\NewDocumentCommand{\subfig}{O{0.2} m o}{%
    \IfValueTF{#3}{%
        \subfloat[#3\label{fig:#2}]{\includegraphics[width=#1\textwidth]{#2}}%
    }{%
        \subfloat{\includegraphics[width=#1\textwidth]{#2}}%
    }%
    \hfil%
}


%% Footnotes
\newcommand{\footnoteErwan}[1]{\footnote{\textcolor{teal}{Erwan: #1}}}

\newcommand{\footnoteurl}[1]{\footnote{\ \url{#1}}}


%% Lists
\renewcommand{\descriptionlabel}[1]{\hspace{\labelsep}\textit{#1}} % Use italics instead of bold for descriptions


%% Maths
\newcommand{\measure}[3]{$\mathrm{#1} = \qty{#2}{#3}$}

\newcommand{\anova}[3]{$\mathrm{F_{#1,#2}} = #3$}

\newcommand{\ci}[2]{$\mathrm{CI_{95\%}}[#1, #2]$}

\newcommand{\friedman}[1]{$\chi^2 = #1$}

\newcommand{\geomean}[2]{\measure{GM}{#1}{#2}}

\newcommand{\iqr}[2]{\measure{IQR}{#1}{#2}}

\newcommand{\kruskal}[1]{\measure{H}{#1}{}}

\newcommand{\median}[2]{\measure{Mdn}{#1}{#2}}

\newcommand{\p}[2][=]{$\mathrm{p} #1 \num{#2}$}

\newcommand{\pearson}[1]{\measure{r}{#1}{}}

\newcommand{\tabCI}[2]{{[}#1{,}\,#2{]}}

\newcommand{\wilcoxon}[1]{$V = #1$}


%% References
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\subsecref}[1]{Subsec.~\ref{#1}}


%% Review
\newcommand{\added}[1]{#1}
\newcommand{\removed}[1]{}
\newcommand{\replaced}[2]{#2}

\renewcommand{\added}[1]{\textcolor{Blue}{#1}}
\renewcommand{\removed}[1]{\textcolor{Red}{\st{#1}}}
\renewcommand{\replaced}[2]{\removed{#1} \added{#2}}


%% Sections
\newcommand{\subsubsubsection}[1]{\paragraph*{\textit{#1}}}


%% Tables
% example:
% \begin{tab}{label}{Title}{| c | c |}
%     \hline
%     \textbf{1} & \textbf{2} \\ \hline
%       3 & 4 \\ \hline
% \end{tab}
% reference later with: \tabref{label}
\NewDocumentEnvironment{tab}{m m m}{%
    \begin{table}%
        \begin{center}
            \caption{#2}%
            \label{tab:#1}%
            \begin{tabular}{#3}
                \hline
                }{%
            \end{tabular}%
        \end{center}%
    \end{table}%
}

\NewDocumentEnvironment{tabwide}{m m m}{%
    \begin{table*}%
        \begin{center}
            \caption{#2}%
            \label{tab:#1}%
            \begin{tabular}{#3}
                \hline
                }{%
            \end{tabular}%
        \end{center}%
    \end{table*}%
}

\newcommand{\tabrow}[1]{#1 \\ \hline}

\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

